Monitoring Targeted Hate in Online Environments

Hateful comments, swearwords and sometimes even death threats are becoming a reality for many people today in online environments. This is especially true for journalists, politicians, artists, and other public figures. This paper describes how hate directed towards individuals can be measured in online environments using a simple dictionary-based approach. We present a case study on Swedish politicians, and use examples from this study to discuss shortcomings of the proposed dictionary-based approach. We also outline possibilities for potential refinements of the proposed approach.

==> std_table_ws3.tex <==
\begin{table*}
\begin{tabular}{l l l l l l l}
\bf{Name}& \bf{Anger}& \bf{Naughtiness}& \bf{Swearword} & \bf{General threat}& \bf{Death threat} & \bf{Sexism} \\
\hline
Stefan Löfven&$0.00197$&$0.00178$&$0.00216$&$0.00141$&$0.00009$&$0$\\
Morgan Johansson&$0.00127$&$0.00064$&$0.00223$&$0.00191$&$0.00064$&$0$\\
Margot Wallström&$0.00186$&$0.00149$&$0.00112$&$0.00037$&$0$&$0$\\
Magdalena Andersson&$0.00104$&$0.00104$&$0.00052$&$0.00207$&$0$&$0$\\
Ylva Johansson&$0.00066$&$0.00131$&$0.00197$&$0$&$0$&$0$\\
Gustav Fridolin&$0$&$0.0027$&$0.0018$&$0.0009$&$0$&$0$\\
Alice Bah Kuhnke&$0$&$0$&$0.00176$&$0$&$0$&$0$\\
Peter Eriksson&$0$&$0$&$0$&$0$&$0$&$0$\\
Peter Hultqvist&$0.00439$&$0$&$0$&$0.00439$&$0$&$0$\\
Isabella Lövin&$0$&$0$&$0$&$0$&$0.0054$&$0$\\
Mikael Damberg&$0.00592$&$0$&$0$&$0$&$0$&$0$\\
Ardalan Shekarabi&$0$&$0.00633$&$0$&$0$&$0$&$0$\\
Åsa Regnér&$0$&$0$&$0$&$0$&$0$&$0$\\
Ann Linde&$0$&$0$&$0$&$0$&$0$&$0$\\
Annika Strandhäll&$0$&$0$&$0.1122$&$0$&$0$&$0$\\
Ibrahim Baylan&$0$&$0$&$0$&$0$&$0$&$0$\\
Per Bolund&$0$&$0$&$0$&$0$&$0$&$0$\\
Anna Ekström&$0$&$0$&$0$&$0$&$0$&$0$\\
Heléne Fritzon&$0$&$0$&$0$&$0$&$0$&$0$\\
Tomas Eneroth &$0$&$0$&$0.04167$&$0$&$0$&$0$\\
Helene Hellmark Knutsson&$0$&$0$&$0$&$0$&$0$&$0$\\
Karolina Skog&$0$&$0$&$0$&$0$&$0$&$0$\\
Sven-Erik Bucht&$0$&$0$&$0$&$0$&$0$&$0$\\
\hline
$\mu$&$0.00074$&$0.00066$&$0.00719$&$0.00048$&$0.0054$&$0$\\
$\sigma$&$0.0015$&$0.00141$&$0.02392$&$0.00104$&$0.0011$&$0$\\

\end{tabular}
\label{tab:stats}
\caption{Absolute difference between window size 3 and 5}
\end{table*}


%%
%\begin{table*}
%\begin{tabular}{l l l l l l l}
%\bf{Name}& \bf{Anger}& \bf{Naughtiness}& \bf{Swearword} & \bf{General threat}& \bf{Death threat} & \bf{Sexism} \\
%\hline
%Stefan Löfven & 26 & 49 & 16 & 7 & 0 & 0\\
%Morgan Johansson & 9 & 14 & 3 & 5 & 0 & 0\\
%Margot Wallström & 10 & 11 & 5 & 1 & 0 & 0\\
%Ylva Johansson & 3 & 3 & 5 & 1 & 0 & 0\\
%Gustav Fridolin & 2 & 4 & 3 & 1 & 0 & 0\\
%Magdalena Andersson & 0 & 2 & 1 & 0 & 0 & 0\\
%Mikael Damberg & 1 & 0 & 1 & 0 & 0 & 0\\
%Peter Eriksson & 1 & 0 & 1 & 0 & 0 & 0\\
%Alice Bah Kuhnke & 0 & 0 & 1 & 0 & 0 & 0\\
%Ann Linde & 0 & 0 & 0 & 1 & 0 & 0\\
%Isabella Lövin & 0 & 1 & 0 & 0 & 0 & 0\\
%Magdalena Johansson & 0 & 0 & 0 & 0 & 0 & 0\\
%Peter Hultqvist & 0 & 0 & 0 & 0 & 0 & 0\\
%Ibrahim Baylan & 0 & 0 & 0 & 0 & 0 & 0\\
%Ardalan Shekarabi & 0 & 0 & 0 & 0 & 0 & 0\\
%Per Bolund & 0 & 0 & 0 & 0 & 0 & 0\\
%Karolina Skog & 0 & 0 & 0 & 0 & 0 & 0\\
%Sven-Erik Bucht & 0 & 0 & 0 & 0 & 0 & 0\\
%Åsa Regnér & 0 & 0 & 0 & 0 & 0 & 0\\
%Anna Ekström & 0 & 0 & 0 & 0 & 0 & 0\\
%Helene Hellmark Knutsson & 0 & 0 & 0 & 0 & 0 & 0\\
%Annika Strandhäll & 0 & 0 & 0 & 0 & 0 & 0\\
%Heléne Fritzon & 0 & 0 & 0 & 0 & 0 & 0\\
%
%\end{tabular}
%\label{table:names}
%\caption{Standard deviations for each category for each minister}
%\end{table*}

